CFD-DEM study of mixing in a monodispersed solid-liquid fluidized bed

In this work, we assess the internal dynamics of particles in liquid-solid fluidized beds using an unresolved CFD-DEM model. We use the Nearest Neighbors Method (NNM) and the mixing index based on the principal component analysis proposed by Doucet et al. [1] to quantify the bed mixing for several flow regimes and particle properties. Discussions on the advantages and drawbacks of each method are provided. Using results for several inlet flow rates, we show that the dimensionless mixing time reaches a plateau and does not increase significantly with the inlet velocity. The principal component analysis shows that the studied fluidized bed has no preferential mixing component. Additionally, we show that, except for the sliding friction coefficient, the collision properties have almost negligible influence on the mixing behavior.

==> src/macros.tex <==
%*************************
% Vectors and scalars
%*************************
\newcommand{\Reu}{\mathrm{Re}}
\newcommand{\Rep}{\mathrm{Re}_{p,i}}
\newcommand{\uu}{\bm{u}}
\newcommand{\uej}{\bm{u}_{e,j}}
\newcommand{\ueij}{\bm{u}_{e,ij}}
\newcommand{\bcu}{\left. \bm{u} \right |_{\Gamma_u}}
\newcommand{\vv}{\bm{v}}
\newcommand{\nabu}{\nabla \bm{u}}
\newcommand{\nabdu}{\nabla \cdot \bm{u}}
\newcommand{\uxu}{\bm{u} \otimes \bm{u}}
\newcommand{\vi}{\bm{v}_i}
\newcommand{\wi}{\bm{\omega}_{i}}
\newcommand{\xii}{\bm{x}_i}
\newcommand{\moi}{I_i}
\newcommand{\ident}{\bm{\mathcal{I}}}
\newcommand{\tor}[2]{\bm{M}_{#1, #2}}
\newcommand{\rel}{\left ( \bm{u} - \bm{v}_i \right )}
\newcommand{\relp}{\bm{v}_{rel,ij}}
\newcommand{\relpn}{\bm{v}_{n,ij}}
\newcommand{\relpt}{\bm{v}_{t,ij}}
\newcommand{\pns}{\nabla p}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\tauns}{\nabla \cdot \bm{\tau}}
\newcommand{\eps}{\varepsilon_f}
\newcommand{\beps}{\bar{\varepsilon}_{f}}
\newcommand{\mass}{m_i}
\newcommand{\f}[1]{\bm{f}_{#1}}
\newcommand{\fii}[1]{\bm{f}_{#1,i}}
\newcommand{\fij}[1]{\bm{f}_{#1,ij}}
\newcommand{\fik}[2]{\bm{f}_{#1,#2}}
\newcommand{\FA}[1]{\bm{F}_{#1}^A}
\newcommand{\FB}[1]{\bm{F}_{#1}^B}
\newcommand{\domain}{V_{\Omega}}
\newcommand{\Nn}{N_{nodes}}
\newcommand{\xej}{\bm{x}_{e,j}}
\newcommand{\bcx}[1]{\left. \bm{x} \right |_{#1}}
\newcommand{\tei}{T_{e,i}}
\newcommand{\psii}{\psi_{e,i}}
\newcommand{\tej}{T_{e,j}}
\newcommand{\psij}{\psi_{e,j}}
\newcommand{\phij}{\varphi_{e,j}}
\newcommand{\matA}{\bm{\mathrm{A}}}
\newcommand{\matM}{\bm{\mathrm{M}}}
\newcommand{\vecQ}{\mathrm{Q}}
\newcommand{\vecF}{\mathrm{F}}
\newcommand{\vecu}{\bm{\mathrm{u}}}
\newcommand{\vecud}{\bm{\mathrm{\dot{u}}}}
\newcommand{\vecT}{\mathrm{T}}
\newcommand{\vecTt}{\mathrm{\dot{T}_e}}
\def\Real{\mathrm{I\!R}}

%***************************
% Diferentials
%***************************
\newcommand{\ddp}[2]{\frac{\partial}{\partial #2}\left(#1\right)}
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddt}[1]{\frac{\partial #1}{\partial t}}
\newcommand{\DD}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\newcommand{\DDP}[2]{\frac{\mathrm{d}}{\mathrm{d} #2}\left(#1\right)}
\newcommand{\DDt}[1]{\frac{\mathrm{d} #1}{\mathrm{d} t}}

%***************************
% Integration
%***************************
\newcommand{\ts}{\Delta t}

%****************************************
% Enclosers
%****************************************
\newcommand{\bra}[1]{\left[#1\right]}
\newcommand{\pp}[1]{\left(#1\right)}
\newcommand{\norm}[1]{\left|#1\right|}
\newcommand{\curly}[1]{\left \{ #1 \right \}}
\newcommand{\ens}[1]{\left\langle #1\right\rangle}
\newcommand{\underb}[2]{\underbrace{#1}_{\textup{#2}}}


%****************************************
% Pairs
%****************************************
\newcommand{\normal}{\bm{n}_{ij}}
\newcommand{\nolp}{\delta_{n,ij}}
\newcommand{\tolp}{\delta_{t,ij}}
\newcommand{\nij}[1]{#1_{n,ij}}
\newcommand{\tij}[1]{#1_{t,ij}}

